Split-kl and PAC-Bayes-split-kl Inequalities for Ternary Random Variables

We present a new concentration of measure inequality for sums of independent bounded random variables, which we name a split-kl inequality. The inequality is particularly well-suited for ternary random variables, which naturally show up in a variety of problems, including analysis of excess losses in classification, analysis of weighted majority votes, and learning with abstention. We demonstrate that for ternary random variables the inequality is simultaneously competitive with the kl inequality, the Empirical Bernstein inequality, and the Unexpected Bernstein inequality, and in certain regimes outperforms all of them. It resolves an open question by Tolstikhin and Seldin [2013] and Mhammedi et al. [2019] on how to match simultaneously the combinatorial power of the kl inequality when the distribution happens to be close to binary and the power of Bernstein inequalities to exploit low variance when the probability mass is concentrated on the middle value. We also derive a PAC-Bayes-split-kl inequality and compare it with the PAC-Bayes-kl, PAC-Bayes-Empirical-Bennett, and PAC-Bayes-Unexpected-Bernstein inequalities in an analysis of excess losses and in an analysis of a weighted majority vote for several UCI datasets. Last but not least, our study provides the first direct comparison of the Empirical Bernstein and Unexpected Bernstein inequalities and their PAC-Bayes extensions.

==> checklist.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section*{Checklist}


%%% BEGIN INSTRUCTIONS %%%
\iffalse
The checklist follows the references.  Please
read the checklist guidelines carefully for information on how to answer these
questions.  For each question, change the default \answerTODO{} to \answerYes{},
\answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
justification to your answer}, either by referencing the appropriate section of
your paper or providing a brief inline description.  For example:
\begin{itemize}
  \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
  \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
  \item Did you include the license to the code and datasets? \answerNA{}
\end{itemize}
Please do not modify the questions and only use the provided macros for your
answers.  Note that the Checklist section does not count towards the page
limit.  In your paper, please delete this instructions block and only keep the
Checklist section heading above along with the questions/answers below.
\fi
%%% END INSTRUCTIONS %%%


\begin{enumerate}


\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{All assumptions are stated in the statements of the theorems.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{The work mainly discussed the fundamental concentration inequalities and the potential applications. The main applications discussed in the work are PAC-Bayes analysis on classification problems, and the potential negative societal impacts follow the problems being studied.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{}
        \item Did you include complete proofs of all theoretical results?
    \answerYes{}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See Section~\ref{sec:experiments}, Appendix~\ref{app:sec:experiments}.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See Section~\ref{sec:experiments}, Appendix~\ref{app:sec:experiments}.}
        \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{}
        \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{Appendix~\ref{app:sec:experiments}.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{In the code and in the paper.}
  \item Did you mention the license of the assets?
    \answerYes{}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerYes{New code in the supplementary.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNo{We use publicly available datasets from the UCI and LibSVM repositories.} 
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNo{We use publicly available datasets from the UCI and LibSVM repositories. The data does not contain personally identifiable information or offensive content.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{}
\end{enumerate}


\end{enumerate}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> experiment/FWEL_values.tex <==
\begin{tabular}{|l|l|l|c|c|c|}
\hline
Dataset & Methods & $\Delta_{\ell}=0$ & $\E_{\rho} [\Delta_{\hat L}(h,h_{S_1},S_2)]$ / $\B(\E_{\rho} [\Delta_L(h,h_{S_1})])$  & $\hat L(h_{S_1},S_2)$ / $\B(L(h_{S_1}))$  & $\E_{\rho} [\Delta^+_{\hat L}(h,h_{S_1},S_2)]$ / $\E_{\rho} [\Delta^-_{\hat L}(h,h_{S_1},S_2)]$ \\
\hline
\multirow{3}{*}{\dataset{Haberman}}&PBkl&98.2 \%&-0.001 / 0.373&0.266 / 0.354& \\
&MGG&98.4 \%&-0.001 / 0.124&0.266 / 0.482& \\
&Skl&99.0 \%&-0.001 / 0.095&0.266 / 0.361&0.004 / 0.005 \\
\hline
\multirow{3}{*}{\dataset{Breast-C}}&PBkl&96.6 \%&0.001 / 0.271&0.071 / 0.108& \\
&MGG&97.3 \%&-0.001 / 0.07&0.071 / 0.15& \\
&Skl&98.0 \%&-0.003 / 0.07&0.071 / 0.111&0.009 / 0.011 \\
\hline
\multirow{3}{*}{\dataset{TicTacToe}}&PBkl&91.9 \%&0.01 / 0.259&0.068 / 0.098& \\
&MGG&93.2 \%&-0.006 / 0.082&0.068 / 0.132& \\
&Skl&93.8 \%&-0.015 / 0.093&0.068 / 0.101&0.024 / 0.038 \\
\hline
\multirow{3}{*}{\dataset{Banknote}}&PBkl&98.0 \%&0.005 / 0.197&0.052 / 0.074& \\
&MGG&98.5 \%&0.003 / 0.038&0.052 / 0.099& \\
&Skl&98.8 \%&0.002 / 0.04&0.052 / 0.076&0.007 / 0.005 \\
\hline
\multirow{3}{*}{\dataset{kr-vs-kp}}&PBkl&95.6 \%&0.018 / 0.172&0.046 / 0.059& \\
&MGG&97.7 \%&0.003 / 0.044&0.046 / 0.076& \\
&Skl&98.1 \%&0.001 / 0.046&0.046 / 0.06&0.01 / 0.009 \\
\hline
\multirow{3}{*}{\dataset{Spambase}}&PBkl&86.5 \%&0.044 / 0.204&0.178 / 0.197& \\
&MGG&91.7 \%&0.013 / 0.094&0.178 / 0.222& \\
&Skl&92.4 \%&0.011 / 0.104&0.178 / 0.198&0.043 / 0.033 \\
\hline
\multirow{3}{*}{\dataset{Mushroom}}&PBkl&99.1 \%&0.008 / 0.098&0.002 / 0.005& \\
&MGG&99.7 \%&0.003 / 0.013&0.002 / 0.008& \\
&Skl&99.7 \%&0.002 / 0.013&0.002 / 0.005&0.003 / 0.0 \\
\hline
\multirow{3}{*}{\dataset{Adult}}&PBkl&94.5 \%&0.007 / 0.063&0.165 / 0.172& \\
&MGG&96.5 \%&0.002 / 0.016&0.165 / 0.181& \\
&Skl&97.4 \%&0.001 / 0.02&0.165 / 0.172&0.013 / 0.013 \\
\hline
\end{tabular}


==> experiment/FW_FWEL_table.tex <==
\begin{tabular}{|l|l|ll|ll|ll|}
\hline
\multirow{2}{*}{Dataset} &  & \multicolumn{2}{c|}{$\PBkl$} & \multicolumn{2}{c|}{$\MGG$} & \multicolumn{2}{c|}{$\Skl$} \\
 & & \multicolumn{1}{c}{$\FW$} & \multicolumn{1}{c|}{$\FWEL$} & \multicolumn{1}{c}{$\FW$} & \multicolumn{1}{c|}{$\FWEL$} & \multicolumn{1}{c}{$\FW$} & \multicolumn{1}{c|}{$\FWEL$} \\
\hline
\multirow{3}{*}{\dataset{Haberman}}&Bound&0.446&0.727&0.469&0.606&0.446&0.456 \\
&Risk&0.27&0.27&0.27&0.27&0.27&0.269 \\
&Var&0.106&0.112&0.106&0.088&0.106&0.044 \\
\hline
\multirow{3}{*}{\dataset{Breast-C}}&Bound&0.16&0.379&0.153&0.22&0.16&0.182 \\
&Risk&0.072&0.075&0.071&0.07&0.071&0.067 \\
&Var&0.112&0.15&0.112&0.1&0.112&0.05 \\
\hline
\multirow{3}{*}{\dataset{TicTacToe}}&Bound&0.144&0.358&0.144&0.214&0.144&0.194 \\
&Risk&0.064&0.089&0.069&0.072&0.064&0.064 \\
&Var&0.005&0.014&0.007&0.008&0.005&0.005 \\
\hline
\multirow{3}{*}{\dataset{Banknote}}&Bound&0.109&0.27&0.102&0.137&0.109&0.115 \\
&Risk&0.06&0.062&0.06&0.06&0.06&0.059 \\
&Var&0.016&0.034&0.016&0.014&0.016&0.008 \\
\hline
\multirow{3}{*}{\dataset{kr-vs-kp}}&Bound&0.101&0.232&0.099&0.12&0.101&0.106 \\
&Risk&0.057&0.068&0.056&0.051&0.056&0.05 \\
&Var&0.006&0.011&0.006&0.004&0.006&0.003 \\
\hline
\multirow{3}{*}{\dataset{Spambase}}&Bound&0.287&0.401&0.298&0.316&0.287&0.302 \\
&Risk&0.199&0.228&0.209&0.189&0.196&0.184 \\
&Var&0.003&0.007&0.004&0.002&0.003&0.002 \\
\hline
\multirow{3}{*}{\dataset{Mushroom}}&Bound&0.016&0.102&0.016&0.021&0.016&0.018 \\
&Risk&0.005&0.011&0.006&0.005&0.005&0.005 \\
&Var&0.002&0.009&0.003&0.003&0.002&0.002 \\
\hline
\multirow{3}{*}{\dataset{Adult}}&Bound&0.193&0.235&0.193&0.197&0.193&0.192 \\
&Risk&0.174&0.179&0.175&0.171&0.175&0.17 \\
&Var&0.002&0.003&0.002&0.001&0.002&0.001 \\
\hline
\end{tabular}


==> experiment/bounds_IP.tex <==
\begin{tabular}{lccc}\toprule
Data set & $\PBKL_{IP}$ & $\MGG_{IP}$ & $\SKL_{IP}$ \\
\midrule
\dataset{Haberman} & 0.754 (0) & 0.619 (0.001) & \textbf{0.463 (0)} \\
\dataset{Breast-C} & 0.388 (0) & 0.22 (0)  & \textbf{0.18 (0)} \\
\dataset{TicTacToe} & 0.365 (0) & 0.211 (0) & \textbf{0.195 (0)} \\
\dataset{Banknote}  & 0.283 (0) & 0.145 (0) & \textbf{0.119 (0)} \\
\dataset{kr-vs-kp}  & 0.232 (0) & 0.117 (0) & \textbf{0.106 (0)} \\
\dataset{Spambase}  & 0.401 (0) & 0.31 (0) & \textbf{0.307 (0)} \\
\dataset{Mushroom}  & 0.108 (0) & 0.023 (0) & \textbf{0.019 (0)} \\
\dataset{Adult}  & 0.243 (0) & \textbf{0.204 (0)} & 0.205 (0) \\
\bottomrule
\end{tabular}

==> experiment/bounds_all.tex <==
\begin{tabular}{lccccccc}\toprule
Data set & $\PBKL_{\pi_0}$ & $\MGG_{\pi_0}$ & $\PBKL_{half}$ & $\MGG_{half}$ & $\PBKL_{IP}$ & $\MGG_{IP}$ & $\SKL_{IP}$ \\
\midrule
\dataset{Haberman} & \textbf{0.395 } & 0.412  & 0.443  & 0.465  & 0.754 & 0.619 & \underline{0.463} \\
\dataset{Breast-C} & 0.151 & \textbf{0.149} & 0.164  & 0.157 & 0.388 & 0.22  & \underline{0.18} \\
\dataset{TicTacToe} & 0.212 & 0.264  & 0.146 & \textbf{0.145} & 0.365 & 0.211 & \underline{0.195} \\
\dataset{Banknote} & 0.132  & 0.134 & 0.112 & \textbf{0.105}  & 0.283 & 0.145 & \underline{0.119} \\
\dataset{kr-vs-kp} & 0.163  & 0.183 & 0.096 & \textbf{0.095}  & 0.232 & 0.117 & \underline{0.106} \\
\dataset{Spambase} & 0.31 & 0.335  & \textbf{0.279} & 0.291  & 0.401 & 0.31 & \underline{0.307} \\
\dataset{Mushroom} & 0.052  & 0.072  & \textbf{0.015} & \textbf{0.015} & 0.108 & 0.023 & \underline{0.019} \\
\dataset{Adult} & 0.233 & 0.241  & \textbf{0.198 } & \textbf{0.198}  & 0.243  & \underline{0.204 } & 0.205  \\
\bottomrule
\end{tabular}

==> experiment/bounds_half.tex <==
\begin{tabular}{lcccc}\toprule
Data set & $\PBKL_{\pi_0}$ & $\MGG_{\pi_0}$ & $\PBKL_{half}$ & $\MGG_{half}$ \\
\midrule
\dataset{Haberman} & \textbf{0.395 (0)} & 0.412 (0) & 0.443 (0.001) & 0.465 (0.001) \\
\dataset{Breast-C} & 0.151 (0) & \textbf{0.149 (0)} & 0.164 (0)  & 0.157 (0) \\
\dataset{TicTacToe} & 0.212 (0) & 0.264 (0) & 0.146 (0) & \textbf{0.145 (0)} \\
\dataset{Banknote} & 0.132 (0)  & 0.134 (0) & 0.112 (0) & \textbf{0.105 (0)} \\
\dataset{kr-vs-kp} & 0.163 (0)  & 0.183 (0) & 0.096 (0) & \textbf{0.095 (0)} \\
\dataset{Spambase} & 0.31 (0) & 0.335 (0) & \textbf{0.279 (0)} & 0.291 (0) \\
\dataset{Mushroom} & 0.052 (0)  & 0.072 (0) & \textbf{0.015 (0)} & \textbf{0.015 (0)} \\
\dataset{Adult} & 0.233 (0) & 0.241 (0) & \textbf{0.198 (0)} & \textbf{0.198 (0)} \\
\bottomrule
\end{tabular}

==> experiment/risks_IP.tex <==
\begin{tabular}{lcccc}\toprule
Data set & $h_S$ & $\PBKL_{IP}$ & $\MGG_{IP}$ & $\SKL_{IP}$ \\
\midrule
\dataset{Haberman} & 0.27 (0) & 0.274 (0.003) & 0.27 (0.003) & \textbf{ 0.269 (0.003)} \\
\dataset{Breast-C} & 0.068 (0) & 0.076 (0) & 0.072 (0) & \textbf{0.07 (0)} \\
\dataset{TicTacToe} & 0.046 (0) & 0.083 (0) & 0.07 (0) & \textbf{0.059 (0)} \\
\dataset{Banknote} & 0.058 (0) & 0.061 (0) & 0.06 (0) & \textbf{ 0.059 (0)} \\
\dataset{kr-vs-kp} & 0.045 (0) & 0.061 (0) & 0.052 (0) & \textbf{0.049 (0)} \\
\dataset{Spambase} & 0.175 (0) & 0.224 (0.001) & 0.187 (0) & \textbf{0.183 (0)} \\
\dataset{Mushroom} & 0.002 (0) & 0.012 (0) & 0.006 (0) & \textbf{0.005 (0)} \\
\dataset{Adult} & 0.168 (0) & 0.178 (0) & 0.172 (0) & \textbf{0.169 (0)} \\
\bottomrule
\end{tabular}

==> experiment/risks_all.tex <==
\begin{tabular}{lcccccccc}\toprule
Data set & $h_S$ & $\PBKL_{\pi_0}$ & $\MGG_{\pi_0}$ & $\PBKL_{half}$ & $\MGG_{half}$ & $\PBKL_{IP}$ & $\MGG_{IP}$ & $\SKL_{IP}$ \\
\midrule
\dataset{Haberman}  & 0.27 & 0.274  & 0.278  & 0.272 & 0.273 & 0.274 & 0.27 & \textbf{\underline{ 0.269}} \\
\dataset{Breast-C} & 0.068 & 0.074  & 0.074  &  0.073  & 0.074 & 0.076 & 0.072 & \textbf{\underline{0.07}} \\
\dataset{TicTacToe} & 0.046 & 0.057  & 0.076 & 0.065 & 0.069 & 0.083  & 0.07  & \textbf{\underline{0.059}} \\
\dataset{Banknote} & 0.058 & 0.06 & 0.061 & 0.06  & 0.06 & 0.061  & 0.06  & \textbf{\underline{0.059}} \\
\dataset{kr-vs-kp} & 0.045 & 0.053   & 0.061  & 0.052 & 0.053 & 0.061  & 0.052  & \textbf{\underline{0.049}} \\
\dataset{Spambase} & 0.175 & 0.183 & \textbf{0.18} & 0.196 & 0.203 & 0.224 & 0.187  & \underline{0.183 } \\
\dataset{Mushroom} & 0.002 & 0.008  & 0.016   & \textbf{0.005} & 0.006 & 0.012  & 0.006  & \textbf{\underline{0.005}} \\
\dataset{Adult} & 0.168  & 0.176 & 0.176 & 0.175 & 0.175 & 0.178 & 0.172 & \textbf{\underline{0.169}} \\
\bottomrule
\end{tabular}

==> experiment/risks_half.tex <==
\begin{tabular}{lcccc}\toprule
Data set & $\PBKL_{\pi_0}$ & $\MGG_{\pi_0}$ & $\PBKL_{half}$ & $\MGG_{half}$ \\
\midrule
\dataset{Haberman} & 0.274 (0.002) & 0.278 (0.002) & \textbf{0.272 (0.003)} & 0.273 (0.003) \\
\dataset{Breast-C} & 0.074 (0) & 0.074 (0) & \textbf{ 0.073 (0)}  & 0.074 (0) \\
\dataset{TicTacToe} & 0.057 (0) & 0.076 (0)  & \textbf{0.065 (0)} & 0.069 (0) \\
\dataset{Banknote} & \textbf{0.06 (0)} & 0.061 (0) & \textbf{0.06 (0)} & \textbf{0.06 (0)} \\
\dataset{kr-vs-kp} & 0.053 (0)  & 0.061 (0) & \textbf{0.052 (0)} & 0.053 (0) \\
\dataset{Spambase} & 0.183 (0) & \textbf{0.18 (0)} & 0.196 (0) & 0.203 (0) \\
\dataset{Mushroom} & 0.008 (0)  & 0.016 (0)  & \textbf{0.005 (0)} & 0.006 (0) \\
\dataset{Adult} & 0.176 (0) & 0.176 (0) & \textbf{ 0.175 (0)} & \textbf{0.175 (0)} \\
\bottomrule
\end{tabular}
